LookupFFN: Making Transformers Compute-lite for CPU inference

While GPU clusters are the de facto choice for training large deep neural network (DNN) models today, several reasons including ease of workflow, security and cost have led to efforts investigating whether CPUs may be viable for inference in routine use in many sectors of the industry. But the imbalance between the compute capabilities of GPUs and CPUs is huge. Motivated by these considerations, we study a module which is a workhorse within modern DNN architectures, GEMM based Feed Forward Networks (FFNs), and assess the extent to which it can be made compute- (or FLOP-) lite. Specifically, we propose an alternative formulation (we call it LookupFFN) to GEMM based FFNs inspired by the recent studies of using Locality Sensitive Hashing (LSH) to approximate FFNs. Our formulation recasts most essential operations as a memory look-up, leveraging the trade-off between the two resources on any platform: compute and memory (since CPUs offer it in abundance). For RoBERTa language model pretraining, our formulation achieves similar performance compared to GEMM based FFNs, while dramatically reducing the required FLOP. Our development is complemented with a detailed hardware profiling of strategies that will maximize efficiency -- not just on contemporary hardware but on products that will be offered in the near/medium term future. Code is avaiable at \url{https://github.com/mlpen/LookupFFN}.

==> inserts/op_count_table.tex <==

\begin{table}[!htbp]
\begin{center}
\begin{scriptsize}
\setlength{\tabcolsep}{5pt}
\begin{tabular}{l|cccccc|ccccc}
\toprule 
Method & MulAdd & Rehash \\
\midrule 
MLP & $n (d + d')$ & no \\
SLIDE & $\tau h d + |S| (d + d')$ & yes \\
MONGOOSE & $\tau h d + |S| (d + d')$ & yes \\
Lookup ($k = 0$) & $\tau h d + h d'$ & no \\
Lookup ($k = 1$) & $\tau h d + (\tau + 1) h d'$ & no \\
\bottomrule
\end{tabular}
\end{scriptsize}
\end{center}
\vspace{-0.1in}
\caption{Operation Counts. $h$ is the number of hash tables. $\tau$ is the length of hash code. $d, n, d'$ are input dimension, hidden dimension, and output dimension. }
\label{tab:op_count}
\vspace{-0.1in}
\end{table}

==> sections/intro-scratch-karu.tex <==
CPU-based inference in data-center is growing in importance as evidenced by recent server chip announcements from IBM~\cite{10.1145/3470496.3533042,intel-amx,9731107} and academic efforts~\cite{usenixatc19,9410437}. The technical and business motivations are latency, security, privacy and the fact that modern data-intensive workloads have AI tasks embedded in a deep pipeline of tasks. CPU chips however lack the computational intensity of raw-FLOPS compared to GPUs, but instead provide tremendously large caches in the range of 128MB to 192MB, and even larger. Further-more, such caches made out SRAMs are more than an order of magnitude more energy efficient to access compared to DRAMs (DDR, GDDR, or HBM)~\cite{google-tpu,horowitz-paper}, while providing $4\times$ access bandwithd~\cite{AMD Zen2 for example, allows 64 bytes per cycle into each core: with 32 cores running 3.2 GHz that amounts 6 TB/sec}. In this context, this paper revisits one of the fundamental building blocks of modern deep-learning: the feed forward network, to examine algorithmic optimizations to make it CPU friendly.

Feed-forward networks are essential components of almost all deep neural networks, such as convolutional networks or Transformers. 
They heavily rely on General Matrix Multiply (GEMM), which is extremely compute intensive, especially for large scale neural networks. Consider a BERT-like transformer configuration, the feed-forward network using GEMMs needs 16X more computation (FLOPS) compared to an idealized lookup technique that sums up the relevant weights alone.
A number of efficient alternatives \cite{??} have been proposed to reduce the FLOPS requirement of feed-forward network. 
One popular line of works try to use Locality Sensitive Hashing (LSH) to address the computational bottleneck of feed-forward via adaptive sparsity. 
For example, Slide \cite{slide} uses LSH to retrieve a small subset of neurons that omit high activation via maximum inner product search (MIPS) and only compute the outputs of these neurons, resulting a sparse network. However, it is known issue that LSH is inefficient in deep learning context. 
Due to the constantly evolving parameters during training, the hash tables need to be constantly updated to adapt for the updated parameter matrices (rehash). Due to the randomness of hash functions, a large number of hash functions are needed to good MIPS results.
Also, the skewed hash bucket distribution makes LSH-based feed-forward networks harder to be parallelized since the computational load of different inputs can be highly different. 

Mongoose \cite{mongoose} propose a update scheduler learnable hash functions to reduce the frequency of hash table updates and number of hash functions. 
However, the need for rehash is not eliminated and training become challenging as there are two optimizations: one for optimizing learnable hash functions and another for optimizing the deep learning models that uses LSH. Also, skewed bucket distribution is still limiting parallelism of LSH. 
On the other hands, Yoso \cite{yoso} propose a specialized use case of LSH so that the skewness of bucket distribution does not affect the computational load to enable easy parallelism. 
However, rehash and a large number of hash functions cannot be avoided, and its back-propagation is complex and relies on the randomness of its hash functions. 

Motivated by the limitations of the LSH-based feed-forward networks, in this paper, we provide a formulation of end-to-end learnable memory lookup for feed-forward network. 
Specifically, instead of having separated parameter matrices and hash tables for these parameter matrices, we propose to directly view the hash tables as learnable modules. Specially, we adapt the idea described in \cite{yoso} but parameterize the hash functions and hash tables. Then, we view each hash function as a bucket selection problem over the associated hash table and use softmax as a differentiable relaxation of the selection problem. Then, we use a sub-sampled softmax as an efficient approximation to the softmax relaxation. 
Further, to reduce the computational cost of computing projection in hash code computation, we provide an efficient but yet expressive projection based on fast Hadamard transform. 
By using the specialized hash tables similar to \cite{yoso}, the skewness of bucket distribution become irrelevant in our proposed method. Since there is not parameter matrices as in \cite{mongoose, slide}, rehashing can be completely avoided, and the gradient updates are performed directly on the hash functions and hash tables. 
The proposed formulation is back-propagatable, and not special optimization on the hash modules is needed. As a result, it can be a drop-in replacement to the vanilla feed-forward networks. 

With this formulation, the majority operations of feed-forward network are memory lookups. And we estimate \textcolor{red}{16$ \times$} reduction on FLOPS requirement compared to vanilla FFN. When used in a Transformer model, this formulation coupled with \cite{yoso} for self-attention computation can cast the majority of operations in the Transformer to memory accesses. Even though this formulation, requires somewhat large tables (16MB and more), with careful algorithm design, we can make the access somewhat cache-friendly, achieving nearly 80\% of all memory accesses to be cache hits. In practice, this means, we are able to reduce the energy consumption of 80\% of access to SRAMs (14 pj per 64-bit access), vs 300 to 450 pj for DRAM-based access. We show that, one contemporary hardware, we are 30\% faster than Vanilla-FFN. With new technology like 3D caches appearing in CPUs and GPUs, we expect SRAM based bandwidth to increase even further, making LookupFFN integer factors faster as memory technology and packaging improvements continue.



==> sections/tmp.tex <==
While GPU clusters remain the de facto choice for training large deep neural network (DNN) models today, a number of reasons including ease of workflow/deployment, security and cost have led to efforts investigating whether CPUs may be viable platforms for inference in day-to-day use across many sectors of the industry. But the imbalance between the compute capabilities of GPUs and CPUs is huge, which has prompted both specialized hardware enhancements from major vendors as well as evaluating which algorithmic modificationscan make deployment more CPU friendly. Motivated by these considerations, we study a  module which is a workhorse within modern DNN architectures, Feed Forward Networks (FFNs) and assess to what extent it can be made compute- (or FLOP-) lite. Our formulation recasts most essential operations as a memory look-up, leveraging the trade-off between the two resources on any platform: compute and memory (since CPUs offer it in abundance). Our development involves a careful redesign of each operation in a FFN, complemented with a detailed hardware profiling of strategies that will maximize efficiency -- not just on contemporary hardware but on products that will be offered in the near/medium term future. While our use case is CPU inference, our method is differentiable and can be trained in an end-to-end manner via back-propagation, which enables easy training and integration into common DNN models.

==> tables/h_tau_trade_off.tex <==

\begin{table}[!t]
\begin{center}
\begin{scriptsize}
\begin{tabular}{lccccc}
\toprule
$h$ & $\tau$ & Projection Dim & GFLOPS & Log Perplexity \\
\midrule
64 & 4 & 256 & 0.07 / 0.35 & 1.984 \\
32 & 8 & 256 & 0.03 / 0.31 & 1.939 \\
20 & 13 & 260 & 0.02 / 0.30 & 1.874 \\
\bottomrule
\end{tabular}
\end{scriptsize}
\end{center}
\caption{Validation log perplexity when increasing $\tau$ but decreasing $h$ to keep the projection dimension roughly the same. The left value of GFLOPS column is the flop count of weighted accumulation after memory lookup, and the right value is for the entire FFN. }
\label{tab:h_tau_trade_off}
\end{table}

==> tables/num_hashes.tex <==

\begin{table}[!t]
\begin{center}
\begin{scriptsize}
\begin{tabular}{lccccc}
\toprule
$h$ & $\tau$ & Projection Dim & GFLOPS & Log Perplexity \\
\midrule
32 & 8 & 256 & 0.31 & 1.939 \\
64 & 8 & 512 & 0.35 & 1.884 \\
128 & 8 & 1024 & 0.69 & 1.812 \\
256 & 8 & 2048 & 1.38 & 1.739 \\
\bottomrule
\end{tabular}
\end{scriptsize}
\end{center}
\caption{Validation log perplexity when increasing $h$. }
\label{tab:num_hashes}
\end{table}

==> tables/projection_types.tex <==
\begin{table}[!t]
\begin{center}
\begin{scriptsize}
\begin{tabular}{lccccc}
\toprule
Type & Block Size & GFLOPS & Log Perplexity \\
\midrule
Dense & - & 1.05 / 1.18 & 1.794 \\
BH4 & 64 & 0.56 / 0.69 & 1.812 \\
BH4 & 32 & 0.30 / 0.43 & 1.833 \\
BH4 & 16 & 0.17 / 0.30 & 1.851 \\
\bottomrule
\end{tabular}
\end{scriptsize}
\end{center}
\caption{Log perplexity when using different projections for hash code computation. The left value of GFLOPS column is the flop count of projection, and the right value is for the entire FFN. }
\label{tab:projection_types}
\end{table}

